The Augmented Image Prior: Distilling 1000 Classes by Extrapolating from a Single Image

What can neural networks learn about the visual world when provided with only a single image as input? While any image obviously cannot contain the multitudes of all existing objects, scenes and lighting conditions - within the space of all 256^(3x224x224) possible 224-sized square images, it might still provide a strong prior for natural images. To analyze this `augmented image prior' hypothesis, we develop a simple framework for training neural networks from scratch using a single image and augmentations using knowledge distillation from a supervised pretrained teacher. With this, we find the answer to the above question to be: `surprisingly, a lot'. In quantitative terms, we find accuracies of 94%/74% on CIFAR-10/100, 69% on ImageNet, and by extending this method to video and audio, 51% on Kinetics-400 and 84% on SpeechCommands. In extensive analyses spanning 13 datasets, we disentangle the effect of augmentations, choice of data and network architectures and also provide qualitative evaluations that include lucid `panda neurons' in networks that have never even seen one.

==> figures/perclass.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[t][][b]{.48\columnwidth}
        \centering
        \includegraphics[width=1\columnwidth]{figures/acc.png}
        \caption{Per-class validation accuracy vs training time.}
        \label{fig:acc}
    \end{minipage}%
    \hfill
    \begin{minipage}[t][][b]{0.48\columnwidth}
        \centering
        \includegraphics[width=1\columnwidth]{figures/acc_argmax.pdf}
        \caption{Per-class student performance vs frequency of the class being the top-1 prediction of the teacher.
        %during 1 epoch of training.
        }
        \label{fig:freq}
    \end{minipage}
\end{figure}

==> kd-single-image (ICLR 2023)/.vscode/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> kd-single-image (ICLR 2023)/01.intro.tex <==
\section{Introduction}\label{s:intro}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/splash_v4.pdf}
%     \caption{\textbf{Extrapolating from one image.} Heavily augmented patches from a single image are used to train a student (S) to distinguish semantic classes, such as those in ImageNet.
%     % 
%     The student neural network is initialized from scratch and learns from a pretrained teacher (T) via  KL-divergence.
%     Although almost none of the target classes are present in the image, we find performances $>\!59\%$ for classifying into the $1000$ classes of ImageNet-$12$. 
%     % This shows that combining distillation plus augmentations allows for to extrapolate from a single image to a much larger manifold of natural images.
%     \label{fig:splash}}
% \end{figure}

Deep learning has both relied and improved significantly with the increase in dataset sizes. 
In turn, there are many works that show the benefits of dataset scale in terms of data points and modalities used.
Within computer vision, these models trained on ever larger datasets, such as Instagram-1B~\citep{ig1b} or JFT-3B~\citep{dosovitskiy2020vit}, have been shown to successfully distinguish between semantic categories at high accuracies.
In stark contrast to this, there is little research on understanding neural networks trained on \textit{very small} datasets.
%despite the fact that understanding this regime will likely help in better leveraging the large datasets.
% More importantly, 
Why would this be of any interest? 
While smaller dataset sizes allow for better understanding and control of what the model is being trained with, we are most interested in its ability to  provide insights into fundamental aspects of learning:
For example, it is an open question as to what exactly is required for arriving at semantic visual representations from random weights, and also of how well neural networks can extrapolate from their training distribution.
% To study these questions in their purest form, in this paper we go to the extreme end and analyze whether neural networks can learn to extrapolate from a single datum (singular form of data). % move couple lines later
%\footnote{Grammar note: the singular form of \textit{data} is \textit{datum}.}.

While for visual models it has been established that few or no real images are required for arriving at basic features, like edges and color-contrasts~\citep{asano2020a,KataokaACCV2020,bruna2013invariant,olshausen1996emergence}, we go far beyond these and instead ask what the minimal data requirements are for neural networks to learn \textit{semantic categories}, such as those of ImageNet. 
This approach is also motivated by studies that investigate the early visual development in infants, which have shown how little visual diversity babies are exposed to in the first few months whilst developing generalizeable visual systems~\citep{orhan2020self,bambach2018toddler}.
In this paper, we study this question in its purest form, by analyzing whether neural networks can learn to extrapolate from a single datum. 


% In particular, we are interested in analyzing whether neural networks trained on a single datum can learn more than just generic features such as edges or color-contrasts, but instead learn to distinguish, for example, classes of ImageNet. 


However, addressing this question na\"ively runs into the difficulties of i) current deep learning methods, such as SGD or BatchNorm being tailored to large datasets and not working with a single datum and ii) extrapolating to semantic categories requiring information about the space of natural images beyond the single datum.
In this paper, we address these issues by developing a simple framework that recombines \textit{augmentations} and \textit{knowledge distillation}.

First, augmentations can be used to generate a large number of variations from a single image.
This can effectively address issue i) and allow for evaluating the research question on standard architectures and datasets.
This use of data augmentations to generate variety is drastically different to their usual use-case in which transformations are generated to implicitly encode desirable invariances during training.


Second, to tackle the difficulty of providing information about semantic categories in the single datum setting, we opt to use the outputs of a supervisedly trained model in a knowledge distillation (KD) fashion.
While KD~\citep{hinton2015distilling} is originally proposed for improving small models' performance by leveraging what larger models have learned, we re-purpose this as a simple way to provide a supervisory signal about semantic classes into the training process. 


We combine the above two ideas and provide both student and teacher only with augmented versions of a single datum, and train the student to match the teacher's imagined class-predictions of classes -- almost all of which are not contained in the single datum, see~\cref{fig:splash}.
While practical applications do result from our method -- for example we provide results on single image dataset based model compression in the Appendix -- our goal in this paper is analyzing \textit{the fundamental question} of how well neural networks trained from a single datum can extrapolate to semantic classes, like those of CIFAR, SpeechCommands,  ImageNet or even Kinetics.

%%%%%%%%%%%%%%%

% Within the space of all possible images $I$, a single real image $I$ and its augmentations $A(I)$ provide a very informative prior for extrapolating to real images.
%%%%%%%%%%%%%%%


What we find is that despite the fact that the resulting model has only seen a single datum plus augmentations, surprisingly high quantitative performances are achieved: \eg $74$\% on CIFAR-100, $84\%$ on SpeechCommands and $69$\% top-1, single-crop accuracy on ImageNet-12.
We further make the novel observations that our method benefits from high-capacity student and low-capacity teacher models, and that the source datum's characteristics matter -- random noise or less dense images yield much lower performances than dense pictures like the one shown in Figure~\ref{fig:splash}.

In summary, in this paper we make these four main contributions:
\begin{enumerate}
\itemsep-0.3em 
    \item A minimal framework for training neural networks with a single datum using distillation.
    \item Extensive ablations of the proposed method, such as the dependency on the source image, augmentations and network architectures.
    \item Large scale empirical evidence of neural networks' ability to extrapolate on $>\!12$ vision and audio datasets.
    \item Qualitative insights on what and how neural networks trained with a single image learn.
\end{enumerate}

% \todo{[Remove this paragraph if space is limited]}. The rest of the paper is structured as follows. In the next section~\ref{s:related_work} we review prior work on knowledge distillation and learning deep models without original data. In section~\ref{s:method} we present our framework for distillation with single-datum. The section~\ref{s:experiments} provides an extensive evaluation of the proposed method both in quantitative and qualitative manners. Finally, in section~\ref{s:discussion}, we discuss limitations, societal impacts and outlook for future research to conclude the paper.  

%find the difficult that current deep learning methods are tailored for large datasets and cannot easily be trained in any meaningful way from.

% complex/general function learning, but one that needs lots of data. 
% but is it really able to learn more beyond the trianing data or does it only to interpolation?

% The question whether NNs can extrapolate successfully has been analysed in various aspects but mostly toy
% in this paper 

% In turn, vision models obtained by training on these large datasets have become known and recognized as general visual encoders that ``understand'' the semantics of the visual world, as evidenced by strong transfer learning performances.
% While this correlation of increased dataset sizes and visual understanding is strong, it is unclear whether one follows from the other.
% % this generality stems from the shear scale of the training data or is a different phenomenon which only correlates with increasing dataset sizes.


% Put bluntly: if a visual encoder, such as CNN, trained with half of ImageNet still yields a general visual representation,
% what about a CNN that has only even seen a single image?
% Can this CNN still encode semantics of other real world images in a meaningful manner?
% While a visual encoder, trained with half of ImageNet still yields a general visual representation, taking this to the extreme,
% Driven to one extreme, what about the case when the CNN has only ever seen one image, can it still encode semantics of other real world images in a meaningful manner?


==> kd-single-image (ICLR 2023)/02.related.tex <==
\section{Related Work}
\label{s:related_work}
The work presented builds on top of insights from the topics of knowledge distillation and single- and no-image training of visual representations and yields insights into neural networks' ability to extrapolate.

\paragraph{Distillation.}
In the original formulation of knowledge distillation (KD), the goal is to train a typically lower capacity (``student'') model from a pretrained (``teacher'') model in order to surpass the performance of solely training with a label-supervised objective.
% In knowledge distillation (KD), the teacher is generally a fixed pretrained network learned with a massive amount of high-quality data. 
% In contrast, the student is a usually lower capacity network that is guided to mimic the output of the teacher on a specific task. 
% The rich supervisory signal from the privileged teacher model enables a typically more compact student network to learn important aspects of the input that otherwise could not be possible while solely minimizing a supervised objective.
KD has also been explored extensively to train more performant and, or compressed student models from the soft-target predictions of teacher models~\citep{ba2014do,hinton2015distilling,gou2021knowledge,furlanello2018born,czarnecki2017sobolev}.
Similarly, other approaches have also been developed to improve transfer from teacher to student, including sharing intermediate layers' features~\citep{romero2014fitnets}, spatial attention transfer~\citep{zagoruyko2016paying}, similarity preservation between activations of the networks~\citep{tung2019similarity}, contrastive distillation~\citep{tian2019contrastive} or few-shot distillation~\citep{li2020few}. 
KD has also been shown to be an effective approach for learning from noisy labels~\citep{li2017learning}.
%
More recently,~\citet{beyer2021knowledge} conducted a comprehensive empirical investigation to identify important design choices for successful distillation from large-scale vision models. 
In particular, they show that long training schedules, paired with consistent augmentations (including \textit{MixUp}) for both student and teacher, result in better performances. 
% However, the optimization remains a key bottleneck in successfully bridging the performance gap between student and teacher models~\citep{stanton2021does}.
% In the remainder of this section we focus on the specific domain of distilling models without access to the training data.
% for more on knowledge distillation, see~\citep{gou2021knowledge}.

% %WELL-READ STUDENTS LEARN BETTER
% \citep{turc2019well}

\paragraph{Without the training data.}
Distilling knowledge without access to the original training dataset was originally proposed in $2017$~\citep{lopes2017data} and first experiments of leaving out single MNIST classes from the training data were shown in~\citep{hinton2015distilling}.
Yet, this paradigm is gaining importance as many recent advancements have been made possible due to extremely large proprietary datasets that are kept private. 
This has lead to either the sole release of trained models~\citep{clip,ig65m,ig1b} or even more restricted access to only the model outputs via APIs~\citep{gpt3}.
While the original work~\citep{lopes2017data}, still required activation statistics from the training dataset of the network, more recent works do not require this ``meta-data''.
These approaches are typically generation based~\citep{DAFL,ye2020data,Micaelli2019ZeroShotKT,yin2020dreaming} and \eg yield datasets of synthetic images that maximally activate neurons in the final layer of teacher.
% Similarly, in~\citep{yin2020dreaming}, features of pretrained networks are inverted, a large dataset generated and then used for distillation with high accuracies. 
%
Related to this, there are works which conduct ``dataset'' distillation, where the objective is to distill large-scale datasets into much smaller ones, such that models trained on it reach similar levels of performance as on the original data.
These methods generate synthetic images~\citep{wang2018dataset,radosavovic2018data,liu2019ddflow,zhao2021dsa,cai2020zeroq}, labels~\citep{bohdal2020flexible}, or both~\citep{nguyen2021dataset}, but due to their meta-learning nature have only been successfully applied to small-scale datasets.
%
% Finally, the ability to copy models based on API outputs while having access to a dataset with only a partial overlap to the original one has been explored in~\citep{orekondy19knockoff,wang2020neural}, though \citep{orekondy19knockoff} relies on pretrained models.
%
In contrast to GAN- and inversion-based methods, as well as to dataset distillation, our approach does not require the knowledge of the weights and architecture of the teacher model, and instead works with black-box ``API''-style teacher models and much smaller ``datasets'' of just a single datum plus augmentations.
% Compared to model copying, %our research question is fundamentally different and 
% we do not assume access to any meaningfully similar training dataset, nor start with a pretrained model.
This paper follows a radically different goal: We are interested in \textit{analysing} the potential of extrapolating from a single image to the manifold of natural images, for which we choose KD as a well-suited and simple tool.

\paragraph{Prior knowledge in deep learning.}
Finally, this work is related to several works which have analysed the infusion of prior knowledge to the training process. 
For example the prior knowledge contained in neural network architectures~\citep{jarrett2009best,zhou2019deconstructing,sreenivasan2021finding,kim2021visual, baek2021face, ulyanov2018deep} or image augmentations~\citep{xiao2020should}.
In this work, we instead view a single image as a ``prior'' for all other natural images, which to the best of our knowledge has not been explored.


% \paragraph{Neural network extrapolation.}
% Work on extrapolation behavior mostly focuses on MLPs~\citep{extrap1,extrap2,hettiarachchi2005extrapolation} and GNNs~\citep{xu2020neural}.
% For vision models, only model generalization behavior is analysed, \eg, in \citep{reed2021self, zhou2021domain,sariyildiz2021concept}, however this  confounds training data similarity with re-usability of learned features.
% In this work, we instead investigate the extrapolation performance of vision models \textit{in isolation}  -- to the best of our knowledge, for the very first time.


% \paragraph{Single and no-image training of visual representations.}
% Several prior works propose to learn representations with a single training example, such as a single image, while focusing on specific tasks, such as super resolution or  inpainting~\citep{ulyanov2018deep,shocher2018zero}, generative modelling~\citep{shaham2019singan} and tracking~\citep{rodriguez2012maximum}.
% In self-supervised learning, a single image was shown to be enough for pretraining low-level visual representations when combined with strong data augmentations~\citep{asano2020a}.
% Related to this,~\citep{KataokaACCV2020} pretrained deep visual models with images of fractals and~\citep{baradad2021learning} with uninitialized GAN outputs.
% While these lines of work provide a compelling argument and motivation for this paper by demonstrating the potential of augmentations and limited data, our work is both complementary and goes beyond unsupervised pretraining by showing that KD allows us to learn \textit{semantic} categories, such as those of ImageNet, from \textit{one} image.

==> kd-single-image (ICLR 2023)/03.method.tex <==
\section{Method}\label{s:method}
% Any bells-and-whistles will surely improve performance, but would distract from the science.  
% Therefore, we keep our method pure by simply combining two components: i. the single-image ``patchification'' schema of Asano \etal~\citep{asano2020a}, and ii. the knowledge distillation of .
We believe that simplicity is the key to demonstrating and analysing the question of how far a single image can take us. 
We are inspired by recent work of~\citet{asano2020a}, which ``patchifies'' a single-image using augmentations, and the knowledge distillation method presented by~\citet{beyer2021knowledge} and our technical contribution lies in unifying them to a \textit{single-image distillation} framework.


\paragraph{i. Dataset generation.}
In~\citep{asano2020a}, a single ``source'' image is augmented many times to generate a static dataset of fixed size. 
This is done by applying the following augmentations in sequence: cropping, rotation and shearing, and color jittering. For this, we follow their official implementation\footnote{\url{https://github.com/yukimasano/single_img_pretraining}}, and do not change any hyperparameters. We do however analyze the choice of source images more thoroughly by additionally including a random noise, and a Hubble-telescope image to our analysis. In addition, we also conduct experiments on audio classification. For generating a dataset of augmented audio-clips, we apply the set of audio-augmentations from~\citep{bitton2021augly}, which consist of operations, such as random volume increasing, background noise addition and pitch shifting to yield log-Mel spectrograms from raw waveforms (see Appendix for complete details). 

\paragraph{ii. Knowledge distillation.}
% We do function matching..(introduce network $\Phi$ etc.)
% and also explore effect of cutmix vs mixup.
% however, we do not have access to TPUs and cannot train 10K imagenet epochs.

The knowledge distillation objective is proposed in~\citep{hinton2015distilling} to transfer the knowledge of a pretrained teacher to a lower capacity student model. 
In this case, the optimization objective for the student network is a weighted combination of dual losses: a standard supervised cross-entropy loss and a ``distribution-matching'' objective that aims to mimic the teacher's output.
However, in our case there are no class-labels for the patches generated from a single image, so we solely use the second objective formulated as a Kullback–Leibler (KL) divergence between the student output $p^s$ and the teacher's output $p^t$:
\begin{align}
\label{eq}
    % \mathcal{L}_s &= \alpha \mathcal{L}_{\text{CE}} + (1 - \alpha) \mathcal{L}_{\text{KD}}, \\
    % &\text{with }
%   \mathcal{L}_{\text{CE}} = -\sum_{c ~\in ~\mathcal{C}} y_c\log\sigma_c({l_s}) \\
%   & \qquad 
%   \mathcal{L}_{\text{KD}} = -\tau^2 \sum_{c ~\in ~\mathcal{C}} \sigma_c({l_t}/\tau) \log \sigma_c({l_s}/\tau)    
   \mathcal{L}_{\text{KL}} = \sum_{c ~\in ~\mathcal{C}} -p^{t}_c \log p^{s}_c +p^{t}_c \log p^{t}_c
\end{align}
\noindent where $c$ are the teachers' classes and the outputs of both student and teacher are temperature $\tau$ flattened probabilities, $p = \texttt{softmax}(l/\tau)$, that are generated from logits $l$.
% where $\alpha$ is a weighting factor, $\tau$ is a temperature scaling hyperparameter, and $\mathcal{C}$ is a set of classes. ${l_s}$ and ${l_t}$ are the ``logits'' or  unnormalized outputs of the student and teacher models, respectively. Following~\citep{beyer2021knowledge}, we use $\alpha = 0$, i.e., we do not utilize $\mathcal{L}_{\text{CE}}$ between dataset's hard labels and student model outputs. 

% as shown in~\citep{beyer2021knowledge}, the cross-entropy loss is not esse
% The cross-entropy loss between student outputs $y_s$ and task-specific one-hot labels $y$, and Kullback–Leibler (KL) divergence objective between student and a teacher model output $y_t$ to make student outputs as similar to the teachers as possible. 
% The standard objective widely used for distillation is:
For training, we follow~\citep{beyer2021knowledge} in employing a function matching strategy, where the teacher and student models are fed consistently augmented instances, that include heavy augmentations, such as \textit{MixUp}~\citep{zhang2018mixup} or \textit{CutMix}~\citep{yun2019cutmix}.
%
%
% in providing the student with   signals, \ie providing the student the same augmented samples as the teacher.
% Throughout the paper, we consider a large-scale deep model $\Phi$ (the teacher) with a high performance on a certain task and distill its knowledge with our $1$-image patchification approach to a student network $\phi$ without leveraging any other form of supervision. 
However, in contrast to~\citep{beyer2021knowledge}, we neither have access to TPUs nor can train $10$K epochs on ImageNet-sized datasets.
While both of these would likely improve the quantitative results, we believe that this handicap is actually blessing in disguise: This means that the results we show in this paper are not specific to heavy-compute, or extremely large batch-sizes, but instead are fundamental.

% Howeverbut instead train 200 epochs. 
% In particular, we employ function matching strategy~\citep{beyer2021knowledge}, where, the teacher and student models are feed consistently augmented instances, including image manifold extension via \textit{mixup} or \textit{cutmix} augmentations. We however, do not have access to TPUs and given our modest computational budget use a more relaxed definition of ``patient'' teacher, i.e., we cannot training for $10$k ImageNet epochs. 


==> kd-single-image (ICLR 2023)/04.experiments.tex <==
\section{Experiments}
\label{s:experiments}
\subsection{Implementation details}
\paragraph{Source data.} For the source data, we utilize the single images of~\citep{asano2020a}, except for one image, which we replace by a similar one as we could not retrieve its licence. 
These images are of sizes up to 2{,}560x1{,}920 (the ``City'' image of \cref{fig:splash}).
% In addition, we collect one satellite image of an airport for testing performance in a different remote-sensing domain.
For the audio experiments, we use two short audio-clips from Youtube, a $5$mins BBC newsclip, as well as a $5$mins clip showing $11$ Germanic languages. 
Images and audio visualizations, sources and licences are provided in~\cref{App:viz}.

% \paragraph{Tasks.}
% For simplicity, we focus on classification tasks here and provide results on single-image based model compression in the \cref{appx:data_free_pruning}. 
% For our ablations and small-scale experiments we focus on CIFAR-10/100~\citep{krizhevsky2009learning} and also on the different domain of satellite image classification with the EuroSAT dataset~\citep{helber2019eurosat}.
% For larger-scale experiments using $224\! \times \! 224$ sized images we evaluate our method on datasets with varying number of classes (see \cref{tab:larger-scale}): STL-10~\citep{pmlr-v15-coates11a}, Pets~\citep{parkhi12a}, ImageNet-100~\citep{tian2019contrastive}, Flowers~\citep{Nilsback06}, Places365~\citep{zhou2017places} and finally ImageNet LSVRC12 (IN-1k)~\citep{deng2009imagenet}.
% For our audio experiments in \cref{tab:audio}, we use MUSAN~\citep{snyder2015musan}, Voxforge~\citep{maclean2018voxforge}, SpeechCommands~\citep{warden2018speech}, and LibriSpeech~\citep{panayotov2015librispeech} datasets for varying complexity and categories of sounds to be recognized.

% , and Nsynth~\citep{engel2017neural}
\paragraph{Tasks.}
For simplicity, we focus on classification tasks here and provide results on a sample application of single-image based model compression in \cref{appx:data_free_pruning}. 
For our ablations and small-scale experiments we focus on CIFAR-10/100~\citep{krizhevsky2009learning}. % and also on the different domain of satellite image classification with the EuroSAT dataset~\citep{helber2019eurosat}.
For larger-scale experiments using $224\! \times \! 224$ sized images, we evaluate our method on datasets with varying number of classes (see \cref{tab:larger-scale}) and additionally conduct experiments in the audio domain (see \cref{tab:audio}) and video (see \cref{tab:larger-scale-video}).
Further implementation details are provided in~\cref{App:impl}.

%STL-10~\citep{pmlr-v15-coates11a}, Pets~\citep{parkhi12a}, ImageNet-100~\citep{tian2019contrastive}, Flowers~\citep{Nilsback06}, Places365~\citep{zhou2017places} and finally ImageNet LSVRC12 (IN-1k)~\citep{deng2009imagenet}.
% For our audio experiments in \cref{tab:audio}, we use MUSAN~\citep{snyder2015musan}, Voxforge~\citep{maclean2018voxforge}, SpeechCommands~\citep{warden2018speech}, and LibriSpeech~\citep{panayotov2015librispeech} datasets for varying complexity and categories of sounds to be recognized.
% For our experiments on learning video models from a single image we use the Kinetics-400~\citep{carreira2017quo} and UCF-101~\citep{soomro2012ucf101} datasets.

% \paragraph{Optimization.}
% For each of these datasets, we first train a teacher network in a usual supervised manner, that is then used for the distillation. 
% For the distillation to the student model, we use a temperature $\tau=8$ motivated by findings in~\citep{beyer2021knowledge}.  
% We keep this temperature fixed throughout the whole of the paper due to limited compute.
% For optimization, we use AdamW~\citep{loshchilov2018decoupled}. 
% Further implementation details are provided in~\cref{App:impl}.


\subsection{Ablations}
\begin{table}[]
    \centering
    \begin{minipage}{.6\textwidth}
        \input{tables/_vary_ds}
    \end{minipage}
    \hfill
    \begin{minipage}{.38\textwidth}
    \caption{\textbf{Comparison to other datasets.} Teacher model is WideR40-2 and student is WideR40-1 as in~\citep{Micaelli2019ZeroShotKT}.
            \label{tab:baselines}}
        \setlength{\tabcolsep}{6pt}
          \centering
          \footnotesize
            \begin{tabular}{ll}
            \toprule
            Data & \textbf{C10} \\
            \midrule
            {CIFAR-10} & 92.61 \\
            {Fractals} & 33.26 \\
            {StyleGAN} & 83.42 \\
            {ZeroSKD}  & 86.60\\
            Ours  & 89.27\\
               \bottomrule
            \end{tabular}
    \end{minipage}%
\end{table}


\paragraph{1-image vs full training set.}
We first examine the capability to extrapolate from one image to small-scale datasets, such as CIFAR-10 and CIFAR-100.
In \cref{tab:abl:ds}, we compare various datasets for distilling a teacher model into a student.
We find that while distillation using the source dataset always works best ($95.26\%$ and $78.06\%$) on CIFAR-10/100, using a single image can yield models which almost reach this upper bar ($94.1\%$ and $73.8\%$). 
Moreover, we find that one image distillation even outperforms using $10$K images of CIFAR-10 when teaching CIFAR-100 classes even though these two datasets are remarkably similar.
To better understand why using a single image works, we next disentangle the various components used in the training procedure: (a) the source image, (b) the generated image dataset size and (c) the augmentations used during distillation, corresponding to \cref{tab:abl:image,tab:abl:aug}.

\input{tables/analysis}

% \paragraph{1-image training parameters.}
% From \cref{tab:abl:image}, we find that the choice of source image content is crucial: Random noise or sparser images perform significantly worse compared to the denser ``City'' and ``Animals'' pictures. 
% This is in contrast to self-supervised pretraining analyzed in~\citep{asano2020a}, suggesting that the underlying mechanisms are different.
% Next, from \cref{tab:abl:size}, we find that adding more variation to the initial set of crops improves performance in a progressive manner, where the first $10$x in the number of initial crops adds $4.9$\% in CIFAR-100 performance and the last one only adds 0.9\%.
% While out of scope for this paper, this suggest that there is still room to optimize the initial set of crops used to generate this dataset.
% Finally in \cref{tab:abl:aug}, we ablate the augmentation we use during knowledge distillation. 
% Besides observing the general trend of ``more augmentations are better'', we find that \textit{CutMix} performs better than \textit{MixUp} on our single-image distillation task.
% This might be because in our case the model is tasked with learning how to extrapolate towards real datapoints, while \textit{MixUp} is derived and therefore might be more useful for interpolating between (real) data samples~\citep{zhang2018mixup,beyer2021knowledge}.

\begin{figure}
    \centering
    \noindent\includegraphics[width=\textwidth]{figures/cifar_100_images_ablation.pdf} 
    \caption{\textbf{CIFAR-100 accuracies for varying source images.} Setting as in~\ref{tab:abl:image}.
    \label{fig:vary_image}}
\end{figure}

\paragraph{Choice of single image.}
From \cref{tab:abl:image}, we find that the choice of source image content is crucial: Random noise or sparser images perform significantly worse compared to the denser ``City'' and ``Animals'' pictures. 
We compare 23 further images in~\cref{fig:vary_image} and find that distillation quality roughly correlates with the density in images and JPEG sizes.
This is in contrast to self-supervised pretraining of~\citep{asano2020a}, suggesting that the underlying mechanisms are different.

% Next, from \cref{tab:abl:size}, we find that adding more variation to the initial set of crops improves performance in a progressive manner, where the first $10$x in the number of initial crops adds $4.9$\% in CIFAR-100 performance and the last one only adds 0.9\%.
% While out of scope for this paper, this suggest that there is still room to optimize the initial set of crops used to generate this dataset.


\paragraph{Varying loss functions.} In~\cref{tab:dist_type}, we show that  the student can learn even with much degraded learning signals.
For example even if it receives only the top-5 predictions or solely the argmax prediction (\ie a hard label) of the teacher without any confidence value, the student is still able to extrapolate at a significant level ($>\!91\%/60\%$ for CIFAR-10/100). 
Even at ImageNet scale, the performance remains at a high $43.8\%$ top-1 accuracy (see~\cref{tab:larger-scale} row \textit{(m)}).
This also suggests that copying models solely from API outputs is possible, similar to~\citep{orekondy19knockoff}. 
We also evaluated L1 and L2 distillation functions (see~\cref{tab:appendix_loss_fns} for details) and found that these perform slightly worse. 
This echoes the finding of~\citep{tian2019contrastive} that standard KD loss of \cref{eq} is actually a strong baseline, hence we use this in the rest of our experimental analysis.

\paragraph{Augmentations.}
In \cref{tab:abl:aug}, we ablate the augmentations we use during knowledge distillation. 
Besides observing the general trend of ``more augmentations are better'', we find that \textit{CutMix} performs better than MixUp on our single-image distillation task.
This might be because in our case the model is tasked with learning how to extrapolate towards real datapoints, while MixUp is derived and therefore might be more useful for interpolating \textit{between} (real) data samples~\citep{zhang2018mixup,beyer2021knowledge}.
% Appendix 


% \input{tables/vary_distillation_data}





% \paragraph{1-image vs other datasets.}
% In \cref{tab:baselines}, we find that there is something unique about using a single image, as our method outperforms several synthetic datasets, as well as the GAN-based approach of~\citep{Micaelli2019ZeroShotKT}. 
% This is despite the fact that these synthetic datasets contain $\sim\!50$K images. 
% We provide insights on the characteristics of this 1-image dataset in~\cref{sec:datasetsize}.

\paragraph{Comparison to synthetic datasets.}
In \cref{tab:baselines}, we find that there is something unique about using a single image, as our method outperforms several synthetic datasets, such as FractalDB~\cite{KataokaACCV2020}, randomly initialized StyleGAN~\cite{baradad2021learning}, as well as the GAN-based approach of~\citep{Micaelli2019ZeroShotKT}. 
This is despite the fact that these synthetic datasets contain $\sim\!50$K images. 
We provide insights on the characteristics of this 1-image dataset in~\cref{sec:datasetsize}.
Next, using the insights gained in this section, we scale the experiments towards other network architectures, dataset domains and dataset sizes.

% \todo{(potentially: refer to appendix: experiment with only $100$K teacher queries)
% CIFAR-$10$: 77.45
% CIFAR-$100$: 44.62}

% \paragraph{Teacher signal.}
% In \cref{tab:dist_type}, we also ablate the type of learning signal the student receives.
% We find that even if the student receives only the top-5 predictions, or even just the argmax prediction (\ie, a hard label) of the teacher without any confidence value, the student is still able to extrapolate to CIFAR images at a significant level. 
% While these datasets are small, this might suggest copying larger models from API outputs is possible, similar to~\citep{orekondy19knockoff}.

% Next, using the insights gained in this section, we scale the experiments towards other network architectures, dataset domains and dataset sizes.

\subsection{Generalisation}
\paragraph{Architectures}
\input{tables/vary_archs}
In \cref{tab:architectures}, we experiment with different common architectures on CIFAR-10 and CIFAR-100. 
On CIFAR-10, we find that almost all architectures perform similarly well, except for the case of ResNet-56 to ResNet-20 which could be attributed to the lower capacity of the student model. 
We find that the distillation performance of \mbox{WideR40-4} to WideR40-4 on CIFAR-10 is very close to distilling from original source data; achieving accuracy of $94.14\%$ and only around one-percentage point lower than supervised training. 
This analysis shows that our method generalizes to other architectures hints that larger capacity student models might be important for high performances.    

 
% COMMNETED OUTTTT %%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Varying data domain}
% \input{tables/other_domain}
% We investigate how the proposed single-image distillation performs on varying the data domain. 
% To this end, we focus on satellite imagery classification following the same experimental protocol as before. 
% In \cref{tab:other}, we first report distillation performance when using EuroSAT as the source data for CIFAR-100 and vice versa. 
% The performance on the latter drops significantly to $9.3\%$ when input domain changes as these datasets are largely unrelated and EuroSAT is less diverse. 
% Next, we perform distillation with a single-image datasets generated from an `Animal' and `Satellite-picture' images. 
% To our surprise, we notice significantly high accuracy of $95\%$ even when using completely unrelated data, while combining the data from varying sources equally slightly improves the distillation performance on EuroSAT with only two-percentage point lower accuracy on CIFAR-100.
% From this evaluation, we can conclude that the our distillation framework works equally well on different data domains, and being strictly in-domain is not necessary as long as the image is diverse.

\paragraph{Extension to audio.}
\input{tables/audio}
So far, our proposed approach has shown success in distilling useful knowledge for images. 
To further test the generalizability of our approach on other modalities, we conduct experiments on several audio recognition tasks of varying difficulty. 
We perform distillation via $50$K randomly generated short audio clips from two (\ie $\text{Ours}_A$ and $\text{Ours}_B$), $5$mins YouTube videos (see~\cref{App:viz} for more details). 
In \cref{tab:audio}, we compare the results against the performance of the teacher model and distilling directly using source dataset. 
We find that even for audio, distilling with merely a single audio clip's data provides enough supervisory signal to train the student model to reach above $80\%$ accuracy in the majority of the cases. 
In particular, we see significant improvement in distillation performance when a single audio has a wide variety of sounds to boost accuracy on challenging Voxforge dataset from $72.8\%$ to $78.4\%$.  
Our results on audio recognition tasks demonstrate the modality agnostic nature of our approach and further highlight the capability to perform knowledge distillation in the absence of large amount of data. 


\paragraph{Extension to video.}
We conduct further experiments on video action recognition tasks.
As distillation data, we generate simple pseudo-videos of 12 frames that show a linear interpolation of two crop locations at taken at the beginning and end for the City image and use X3D video architectures~\citep{feichtenhofer2020x3d} as teachers and students, see~\cref{app:video} for further details.
In \cref{tab:larger-scale-video}, we find that our approach indeed generalizes well to distilling video models with performances of 75.2\% and 51.8\% on UCF-101~\citep{soomro2012ucf101} and K400~\citep{carreira2017quo}--despite the fact that the source data is not even a real video.


\begin{table}[]
    \centering
    \begin{minipage}{.36\textwidth}
        \input{tables/video}
    \end{minipage}
    \hfill
    \begin{minipage}{.55\textwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/combined_hist.pdf}
    \captionof{figure}{\textbf{Output confidence scores.} Temperature-scaled softmax scores of the predicted classes for $5$K patches and the $5$K \mbox{CIFAR-10} validation set images.}
    \label{fig:combined_hist}
% \end{figure}
    \end{minipage}%
\end{table}

% \input{tables/video}


\subsection{Scalability to large-scale datasets and models \label{sec:datasetsize}}
\input{tables/larger_scale}
From this section on, we scale our experiments to larger models utilizing 224$\times$224-sized images, and evaluate these on various vision datasets.

\paragraph{Varying datasets.} In~\cref{tab:larger-scale} we find that, overall, a single image is not enough to fully recover the performance on more difficult datasets. 
This might be because of the fine-grained nature of these datasets, \eg ImageNet includes more than $120$ kinds of dogs and Flowers contains $102$ types of flowers.
% Extrapolating from a single image to these very similar categories therefore likely requires a more diverse source image.
Nevertheless, we find a surprisingly high accuracy of $69\%$ on ImageNet's validation set, even though this dataset comprises $1000$ classes, and the student only having seen heavily augmented crops of a single image. 
In \cref{tab:in1k-analysis}, we conduct further analyses on distilling ImageNet models.

\begin{table}[]
    \centering
    \begin{minipage}{.6\textwidth}
    \input{tables/imagenet_analysis}
    \end{minipage}%
    \hfill    
    \begin{minipage}{.36\textwidth}
        \noindent\includegraphics[width=0.99\linewidth]{figures/resnets.pdf} 
        \captionof{figure}{\textbf{Effect of student architecture.} We vary the architecture of the student by depth and width. Teacher is a ResNet-18, settings as in \cref{tab:larger-scale} with half batch size.  \label{fig:size_ablation}}
    \end{minipage}%
\end{table}


\paragraph{Patchification vs more data.} 
At the top part of the \cref{tab:in1k-analysis}, we analyse the effect of using original vs patchified (p) random images from the training set of ImageNet.
We find that while for $10$ and $100$ source images, patchification improves performance, this is not the case when a larger number of images is used. 
This indicates that increased diversity is especially a crucial component for the small data regime, while capturing larger parts of objects becomes important only beyond this stage.
We also make the surprising observation that patches from a single high-quality image (``City'') obtain better performances than patches generated from $1000$ ImageNet training images. 
%
To understand why this might be the case, we note that the high coherency of training patches from a single image strikingly resembles what babies see during their early visual development, \eg, looking at only few toys and people but from many angles~\citep{bambach2018toddler,orhan2020self}.
It is hypothesized that this unique combination of coherence and variability is ideal for learning to recognize objects~\citep{orhan2020self}.


\paragraph{Teacher/student architectures.}
In~\cref{fig:size_ablation}, we analyze the performances of varying ResNet models by depth or width.
We find that overall varying the width is a more parameter-efficient way to obtain higher performances, almost reaching the teacher's $69.5\%$ performance with a ResNet-50x2 at $69.0\%$.


In addition, in the bottom half of \cref{tab:in1k-analysis} (rows \textit{g-n}), we find surprising results:
First, in contrast to normal KD, we find that the teacher's performance is not directly related to the final student performance, \eg a ResNet-50 is less well-suited for distilling than a ResNet-18 (rows \textit{i} vs \textit{l}).

Second, we find that the choice of source image is even more important for ImageNet classification (see rows \textit{g-i}), as switching from the ``City'' even to the ``Bridge'' one decreases performance considerably and the Noise image does not train at all.
Third, we find that the best settings are those in which the student's capacity is higher than that of the teacher (rows \textit{i,n} and \cref{fig:size_ablation}).
% In particular, we can improve from $55.5\%$ top-1 accuracy to $66.2\%$  when switching to a weaker ResNet-18 teacher.
In fact this R18$\rightarrow$R50x2 setup (row \textit{n}) obtains a performance on ImageNet-12 of $69.0\%$ %, which -- though it uses a different architecture and a teacher -- surpasses the ground-breaking AlexNet~\citep{Krizhevsky2012} performance of $56.5\%$ more than $12\%$ and 
which matches the teacher's performance within $0.5\%$.
In~\cref{app:vit}, we further compare distillations to ViT architectures~\citep{dosovitskiy2020vit}, but generally find lower performances (up to 64\%), showing that the inductive biases of CNNs might positively aid in learning.

%% COMMENTED OUT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{tables/representation_exps}
% \paragraph{Representation learning experiments.}
% Given that we can train a ResNet with only a single image and outputs of a pretrained teacher model, it is natural to ask how well this model serves as a \textit{general} visual encoder. 
% For this, we conduct a number of standard representation learning evaluations in \cref{tab:rep} and also compare against running a common self-supervised learning method, MoCo-v2~\citep{he2020momentum}, on the same dataset (see \cref{App:impl} for training and evaluation details).
% We find that freezing the backbone and only training a linear layer on top of it, can achieve performances of $68.7$\% and $47.2$\% for ImageNet and Places, respectively, vastly outperforming the self-supervised variant.
% A similar trend is observed for data-efficient classification.


\subsection{Analysis}
To better understand how our method is achieving these performances, we next analyse the learned models. 
\paragraph{Output confidence scores.}
In \cref{fig:combined_hist}, we visualize the distribution of the confidence scores of the predicted classes for student and teacher models for the training and evaluation data.
We observe that the student indeed learns to mimic the teacher's predictions well for the patch training data.
However, during evaluation on CIFAR images, the student model exhibits a much broader distribution of values, some with extremely high confidence scores. 
This might indicate that the student has learned to identify many discriminative features of object classes from the training data, which are all triggered when shown real examples, leading to much higher confidence values.

\paragraph{Feature space analysis.}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figures/combined_hist.pdf}
%     \caption{\textbf{Output confidence scores.} Temperature scaled softmax scores of the predicted classes for $5$K patches and the $5$K \mbox{CIFAR-10} validation set images.}
%     \label{fig:combined_hist}
% \end{figure}


\input{figures/tsne}
Next, we analyse the network's embedding of training patches when compared to validation-set inputs. 
For this, we fit a $t$-SNE~\citep{van2008visualizing} using the features of $5$K training patches and $5$K test set images in~\cref{fig:cifar_patches_tsne}.
We find that, as expected, the training patches mapped to individual CIFAR classes do not resemble real counter parts.
Moreover, we observe that all the training patches are embedded close to each other in the center, while CIFAR images are clustered towards the outside. 
This shows that the network is indeed learning features that are well suited for effective extrapolation.

\paragraph{Neuron visualizations.}
\input{figures/neurons1}
We next analyze a single-image distilled model trained to predict IN-$1$k classes.
In \cref{fig:neuron}, we visualize four final-layer neurons using the Lucid~\citep{olah2017feature} library. 
When we compare neurons of the standard ImageNet supervised and our distilled model, we find that the neurons activate for very similar looking inputs. 
The clear neuron visualizations for ``panda'' or ``lifeboat'' (and more are provided in~\cref{appendix_s:neuron_activation}) are especially surprising since this network was trained using only patches from the \textit{City} Image, and has never seen any of these objects during its learning phase.


% \paragraph{Per-class evaluations.} 
% \input{figures/perclass}
% We now turn to models trained to predict IN-$1$k classes and analyze per-class performances against training time.
% In~\cref{fig:acc}, we find that the validation performance of IN-1k classes is very diverse: some are identified with  $>\!80\%$ accuracy after just a few epochs of training, such as the class ``Black Swan'', while others require longer training and some are almost impossible to learn, even after $200$ epochs. 
% In \cref{fig:freq}, we plot the validation performance against the frequency of how often the class appears as a top-1 prediction of the teacher during $1$ epoch of training and find that it is unrelated, showing the student is profiting heavily from the knowledge contained in the soft-predictions, echoing findings from~\citep{furlanello2018born,hinton2015distilling}.




==> kd-single-image (ICLR 2023)/05.conclusion.tex <==
\section{Discussion}
\label{s:discussion}
% \todo{In this section, we discuss the limitations and potential negative impact of this work and provide a summary and outlook on the research that this work might enable.} %could leave it out.

\paragraph{The augmented image prior for extrapolation.}
The results in this paper suggest a summary formulation as follows:
\textit{Within the space of all possible images $\mathcal{I}$, a single real image $x\in\mathcal{I}$ and its augmentations $\mathcal{A}(x)$ can provide sufficient diversity for extrapolating to semantic categories in real images.
}


\paragraph{Limitations.}
% In this paper, we were mainly concerned with showing that extrapolating from a single image works, empirically.
% While we do conduct several quantitative and qualitative analyses, we do not provide a theoretical framework but instead believe that theory will follow experimental evidence.
% Due to the limited nature of our compute resources, we have also not extensively analyzed the choice of initial image or patchification augmentations, instead relying on insights from previous works.
In this paper, we were mainly concerned with showing that extrapolating from a single image works, empirically.
% While we do conduct several quantitative and qualitative analyses, we do not provide a comprehensive theoretical framework that explains all of our observations.
%but instead believe that theory will follow experimental evidence.
Due to the limited nature of our compute resources, we have not exhaustively analyzed the choice of initial image or patchification augmentations, and longer training (as shown in~\citep{beyer2021knowledge}) would further improve performances.


% work scratches surface as a lot could be optimized: the choice of image, the choice of initial augmentations and training augmentations and epochs and optimizers.

\paragraph{Potential negative societal impact.}
While our research question is of fundamental nature, one possible negative impact could be that the method is used to steal models and thus intellectual property from API providers --  although in practice the performance varies especially for large-scale datasets (see \cref{tab:larger-scale}).
%study a fundamental research question, we have shown that it is possible to learn behavior from a pretrained teacher model, with only a single datum.
% Thus, it is possible that this method can be used to steal models, although in practice the performance varies widely especially for large-scale datasets (see \cref{tab:larger-scale}).

\paragraph{Conclusion and outlook.}
In this work, we have analyzed whether it is possible to train neural networks to extrapolate to unseen semantic classes with the help of a supervisory signal provided by a pretrained teacher. Our quantitative and qualitative results demonstrate that our novel single-image knowledge distillation framework can indeed enable training networks from scratch to achieve high accuracies on several architectures, datasets and domains. This demonstrates that knowledge distillation can be done with just a single image plus augmentations, and also raises several further research questions, such as the dependency of the source image and the target semantic classes; how networks combine features for extrapolation; and the role and informational content of augmentations; all of which we hope inspires further research
\newpage

==> kd-single-image (ICLR 2023)/figures/cka.tex <==
% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.48\columnwidth}
%     \centering
%     \includegraphics[width=0.92\columnwidth]{figures/cka_wrn16_4_all.pdf}
%     \caption{WideResNet$16\times4$ via CIFAR-10 supervised training vs 1-image distilled.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/cka_r50.pdf}
%     \caption{ResNet50 via ImageNet supervised training vs 1-image distilled.}
%     \end{subfigure}
%     \caption{\textbf{Representation similarity with CKA~\cite{kornblith2019similarity}.} We visualize the similarity between supervised representations and those distilled using random patches of $1-$image. 
%     As in~\cite{nguyen2020wide}, we compute CKA for all the layers in a model using CIFAR-10 testset. The layers in the same block group shows high similarity though both models are trained in different ways, indicating that distilled features are highly similar to those learned in a supervised way.}
%     \label{fig:cka}
% \end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{\columnwidth}
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/cka_wrn16_4_all.pdf}
    \caption{WideR$16-4$ via CIFAR-10 supervised training vs 1-image distilled.}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{\columnwidth}
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/cka_r50.pdf}
    \caption{R50 via ImageNet supervised training vs 1-image distilled.}
    \end{subfigure}
    \caption{\textbf{Representation similarity with CKA~\cite{kornblith2019similarity}.} We visualize the similarity between supervised representations and those distilled using random patches of $1-$image. 
    As in~\cite{nguyen2020wide}, we compute CKA for all the layers in a model using CIFAR-10 testset. The layers in the same block group shows high similarity though both models are trained in different ways, indicating that distilled features are highly similar to those learned in a supervised way.}
    \label{fig:cka}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figures/cka_r50.png}
%     \caption{\textbf{Representation similarity with CKA~\cite{kornblith2019similarity}.} We visualize the similarity between learned representations of ResNet-50 models trained in a supervised manner on ImageNet-12 and one distilled using random patches of $1-$image. We compute CKA for all the layers in a model using $5000$ randomly selected instances from the CIFAR-10 test set (as is done in~\cite{nguyen2020wide}). 
%     %The layers in the same block group shows high similarity though both models are trained in different ways, indicating that distilled features are highly similar to those learned in a supervised way.
%     }
%     \label{fig:ckaIN}
% \end{figure}

==> kd-single-image (ICLR 2023)/figures/neurons1.tex <==
% \begin{figure}
    % \centering
    % \includegraphics[width=\columnwidth]{figures/neurons.pdf}
    % \caption{\textbf{Visualizing neurons} via activation maximisation of final layer neurons. We compare an ImageNet supervisedly trained model against our model which has been trained with single image distillation. Best viewed zoomed-in. We provide further examples in~\cref{appendix_s:neuron_activation}.}
    % \label{fig:neuron}
% \end{figure}

\begin{figure}[tb]
  \begin{minipage}[c]{0.54\textwidth}
    \includegraphics[width=\columnwidth]{figures/neurons.pdf}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.39\textwidth}
    \vspace{1em}
    \caption{\textbf{Visualizing neurons} via activation maximisation of final layer neurons. We compare an ImageNet supervisedly trained model against our model which has been trained with single image distillation. Best viewed zoomed-in. We provide further examples in~\cref{appendix_s:neuron_activation}.}
    \label{fig:neuron}
  \end{minipage}
\end{figure}

==> kd-single-image (ICLR 2023)/figures/perclass.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[t][][b]{.48\columnwidth}
        \centering
        \includegraphics[width=1\columnwidth]{figures/acc.png}
        \caption{Per-class validation accuracy vs training time.}
        \label{fig:acc}
    \end{minipage}%
    \hfill
    \begin{minipage}[t][][b]{0.48\columnwidth}
        \centering
        \includegraphics[width=1\columnwidth]{figures/acc_argmax.pdf}
        \caption{Per-class student performance vs frequency of the class being the top-1 prediction of the teacher.
        %during 1 epoch of training.
        }
        \label{fig:freq}
    \end{minipage}
\end{figure}

==> kd-single-image (ICLR 2023)/figures/tsne.tex <==
\begin{figure}[tb]
  \begin{minipage}[c]{0.39\textwidth}
    \includegraphics[width=\columnwidth]{figures/cifar_patches_tsne.pdf}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.54\textwidth}
    \caption{\textbf{Feature space visualization.} 
    $t$-SNE of jointly embedding random patches ($\cdot$) and CIFAR-$10$ test set ($\times$) instances with our model distilled to classify semantic classes. 
    We also show example images from patches and actual validation set images (enclosed in a box). 
    Note how most training images are contained within a small region while the network needs to extrapolate for the real images which occupy the outer regions in this plot. Best viewed zoomed-in.
    % See Appendix for a similar plot solely for CIFAR-$10$ test set images.
    }
    \label{fig:cifar_patches_tsne}
  \end{minipage}
\end{figure}


==> kd-single-image (ICLR 2023)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> kd-single-image (ICLR 2023)/tables/_vary_augmentation.tex <==
% \begin{table}
\setlength{\tabcolsep}{2pt}
   \centering
   \footnotesize
  \begin{tabular}{cccc cc }
  \toprule
    \multicolumn{4}{c}{\textbf{Augmentations}} &
     \multicolumn{2}{c}{\textbf{Accuracy}}       \\
    Hflip. & RCrop. & MixUp & CutMix & C10 & C100\\
    \midrule 
    \cmark & \cmark & & & 89.34 & 55.05  \\
    \cmark &  & \cmark & & 91.03 & 58.24 \\
    \cmark &  &  & \cmark &  92.86 & 64.26\\
    \hline
    \cmark & \cmark & \cmark & &  92.41 & 63.50 \\
    \cmark & \cmark &  & \cmark &  93.32 & 68.69 \\ % 93.28 & 66.12 \\
    \bottomrule
  \end{tabular}
     \caption{\textbf{Varying Augmentation.} More helps, CutMix is important. \label{tab:abl:aug}}
% \end{table}

==> kd-single-image (ICLR 2023)/tables/_vary_ds.tex <==
% \begin{table}
\setlength{\tabcolsep}{3pt}
   \centering
   \footnotesize
      \caption{\textbf{Distilling dataset.} 1 image + augmentations $\approx$ almost 50K in-domain \underline{C}IFAR-\underline{10}/\underline{100} images. Here, both teacher and student are WideR40-4 networks. \label{tab:abl:ds}}
  \begin{tabular}{l rrrr cc }
  \toprule
   \multicolumn{4}{c}{\textbf{Distillation dataset}} && \multicolumn{2}{c}{\textbf{Accuracy}} \\ 
   \cmidrule{0-3} \cmidrule{6-7}
    Name   & \# Images & \# Pixels & Size (MB)&& C10 & C100 \\
    \midrule 
    CIFAR-10          & 50K & 51M & 145 && 95.26 & 76.29\\
    CIFAR-100         & 50K & 51M & 145 && 94.51 & 78.06\\
    CIFAR-10          & 10K & 10M & 29  && 94.58 & 72.95 \\
    Ours              & 1  & 2.8M & 0.27 && 94.14 & 73.80\\
    \bottomrule
  \end{tabular}
% \end{table}



% \begin{table}
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \footnotesize
%   \caption{\textbf{Distilling dataset.} 1 image + augmentations $\approx$ almost 50K in-domain images. \todo{WRN40x4-WRN40x4} \label{tab:abl:ds}}
%   \begin{tabular}{l rr cc }
%   \toprule
%   \multicolumn{3}{c}{\textbf{Distillation dataset}} & \multicolumn{2}{c}{\textbf{Accuracy}} \\ 
%     Name   & \# Images & \# Pixels & C10 & C100 \\
%     \midrule 
%     CIFAR-10          & 50{,}000 & 51M & 95.26 & 76.29\\
%     CIFAR-100         & 50{,}000 & 51M & 94.51 & 78.06\\
%     CIFAR-10          & 10{,}000 & 10M & 94.58 & 72.95 \\
%     % CIFAR-10          & 3{,}000  & 3.1M  \\
%     Ours              & 1  & 2.8M & 94.14 & 73.80\\
%     \bottomrule
%   \end{tabular}
%   \vspace{2em}
% \end{table}

==> kd-single-image (ICLR 2023)/tables/_vary_image.tex <==
% \begin{table}
\setlength{\tabcolsep}{2pt}
   \centering
   \footnotesize
  \begin{tabular}{l r cc }
  \toprule
   \multicolumn{2}{c}{\textbf{Distillation dataset}} & \multicolumn{2}{c}{\textbf{Accuracy}}\\ 
    Image   & \# Pixels & C10 & C100 \\
    \midrule 
     ``Noise''     & 4.9M & 69.30 & 19.50\\ % random-noise
     ``Universe''  & 4.8M & 88.18 & 39.68\\ % hubble
     ``Bridge''    & 1.1M & 92.24 & 57.87 \\ % sanfrancisco
     ``City''      & 4.9M & 93.13 & 64.85\\ %ameyoko
     ``Animals''   & 2.8M & 93.28 & 66.12 \\ %animals
    \bottomrule
  \end{tabular}
     \caption{\textbf{Distilling image.}  Content of source image matters. \label{tab:abl:image}}
% \end{table}

==> kd-single-image (ICLR 2023)/tables/_vary_source_size.tex <==
% \begin{table}
\setlength{\tabcolsep}{2pt}
   \centering
   \footnotesize
  \def\arraystretch{1.18}
  \begin{tabular}{l r cc }
  \toprule 
   \multicolumn{1}{c}{\textbf{Training}}& \multicolumn{2}{c}{\textbf{Accuracy}} \\
    Size & C10 & C100\\
    \midrule
    % 50    & 1M  & 30.0 & 5.25 \\
    500    & 92.31 & 58.95\\
    5K     & 93.01 & 63.84\\
    50K    & 93.28 & 66.12\\
    500K   & 93.52 & 67.05\\
    \bottomrule
  \end{tabular}
   \caption{\textbf{Source dataset size.} A larger initial pool is better. \label{tab:abl:size}}
% \end{table}

==> kd-single-image (ICLR 2023)/tables/analysis.tex <==

\begin{table*}[tb]
\footnotesize
	\caption{\textbf{Ablations of single image distillation.} We analyze key components in our experimental setup. We report top-1 accuracies for \underline{C}IFAR-\underline{10}/\underline{100}. For the teacher we use WideR40-4 and for the student a WideR16-4 and train for 1K epochs.
% 	(or its equivalent for~\cref{tab:abl:size}). 
	\label{tab:ablation}}
\centering
% 	\begin{subtable}[t]{0.3\linewidth}\centering
% 		{\input{tables/_vary_ds}}
% 	\end{subtable} 
	\begin{subtable}[b]{0.3\linewidth}\centering
		{\input{tables/_vary_image}}
	\end{subtable}
	\hfill
	\begin{subtable}[b]{0.24\linewidth}\centering
\setlength{\tabcolsep}{3.5pt}
  \centering
  \footnotesize
  \begin{tabular}{l cc}
  \toprule 
     & \multicolumn{2}{c}{\textbf{Accuracy}}\\ 
    Signal & C10 & C100 \\
    \midrule 
    Full & 93.32 & 68.69 \\ 
    Top-5 & 92.98 & 64.72 \\
    Argmax & 91.89 & 60.75\\
    \bottomrule
  \end{tabular}
        \caption{\textbf{Teacher signal.} Even with only top-5, or hard distillation, performance only slightly degrades. \label{tab:dist_type}}
\end{subtable}
% 	\begin{subtable}[t]{0.45\linewidth}\centering
% 		{\input{tabs/_vary_ds}}
% 	\end{subtable}
%     \hfill
% 	\begin{subtable}[b]{0.25\linewidth}\centering
% 		{\input{tables/_vary_source_size}}
% 	\end{subtable}
    \hfill
	\begin{subtable}[b]{0.4\linewidth}\centering
		{\input{tables/_vary_augmentation}}
	\end{subtable}
\end{table*}



==> kd-single-image (ICLR 2023)/tables/audio.tex <==
\begin{table}
\setlength{\tabcolsep}{2pt}
   \centering
   \footnotesize
    \caption{\textbf{Distilling audio representations.} $1$ audio clip $+$ augmentations provide stronger supervisory signal for the student to distill teacher's knowledge.
   \label{tab:audio}}
  \begin{tabular}{l l c ccc}
  \toprule
     &&  & \multicolumn{3}{c}{\textbf{Distillation}} \\
     \cmidrule{4-6}
     Dataset& Categories (\#Classes) & Teacher & Full & $\text{Ours}_{A}$ & $\text{Ours}_{B}$\\
    \midrule 
    MUSAN~\citep{snyder2015musan} & Generic sounds (3) &  98.76 & 96.78 & 89.85 & 96.28\\
    Voxforge~\citep{maclean2018voxforge} & Languages (6) & 91.13 & 89.04 & 72.85 & 78.47\\
    Speech Commands~\citep{warden2018speech} & Keywords (12) & 95.15 & 94.86 & 82.90 & 84.19 \\
    LibriSpeech~\citep{panayotov2015librispeech} & Speakers (100) & 99.89 & 99.54 & 78.67 & 84.12\\
    
    % MUSAN & Generic sounds (3) &  98.76 & 96.78 & 89.85 & 96.28\\
    % Voxforge & Languages (6) & 91.13 & 89.04 & 72.85 & 78.47\\
    % Speech Commands & Keywords (12) & 95.15 & 94.86 & 82.90 & 84.19 \\
    % LibriSpeech & Speakers (100) & 99.89 & 99.54 & 78.67 & 84.12\\
    
    
    % Nsynth~\citep{engel2017neural} & Note pitch (128) & 91.65 & 90.40 & 50.59  & 20.83\\
    \bottomrule
  \end{tabular}
\end{table}




==> kd-single-image (ICLR 2023)/tables/imagenet_analysis.tex <==
% \begin{table}
     \caption{\textbf{IN-1k distillations.} We vary distillation dataset and teacher/student configurations. 
   `-' refers to experiments not continued due to compute cost outweighing insights. (p) means images are patchified.
%   `$^\star$' refers to a model trained with many augmentations including RandAugment from~\cite{wightman2021resnet}. 
   `$^\dagger$' refers to models trained with half the batch size due to memory constraints. `AM' refers to only using the argmax as teaching signal.
   \label{tab:in1k-analysis}}
   \vspace{-0.5em}
\setlength{\tabcolsep}{1.5pt}
   \centering
   \footnotesize
  \begin{tabu}{ll lll rrrrr}
  \toprule
   && \multicolumn{3}{c}{\textbf{Setting}}& \multicolumn{5}{c}{\textbf{Epochs}} \\
    &\textbf{Images} & Teacher && Student & 10 & 20 & 30 & 50 & 200 \\ 
    \midrule
    {(a)}&  10 & R50 &$\rightarrow$& R50                                   & 7.6 & 13.3 & - & - &- \\
    {(b)}& 10 (p) & R50 &$\rightarrow$& R50                        & 17.2 & 27.3& - & - &- \\ 
    \midrule
    {(c)}& 100 & R50 &$\rightarrow$& R50        & 14.7 & 25.1 & 32.3 \\
    {(d)}& 100 (p) & R50 &$\rightarrow$& R50                       & 23.6 & 36.1 & 42.8 & - & - \\
    \midrule
    {(e)}&  1000 & R50 &$\rightarrow$& R50                                 & 38.0 & 52.4 & 57.4 & 62.5 & - \\
    {(f)} & 1000 (p) & R50 &$\rightarrow$& R50                      & 27.1 & 39.4 & 45.2 & 50.9 & - \\
    \midrule \midrule
    {(g)}&  Noise (p) & R18 &$\rightarrow$& R50                           & 0.1  & 0.1  & 0.1   & - & - \\
    {(h)}&  Bridge  (p) & R18 &$\rightarrow$& R50                          & 21.2 & 34.8 & 40.0  & - & - \\ 
    {(i)}&  City  (p) & R18 &$\rightarrow$& R50                            & 34.5 & 47.0 & 52.2 & 56.8 & 66.2 \\
    \midrule
    {(j)} & City (p)  & R101 &$\rightarrow^\dagger$& R101                 & 22.4 & 31.4 & - & - & - \\
    % {(h)} & 1x City & WR50-2 &$\rightarrow^\dagger$ & WR50-2            & 29.1 & 39.9 & - & - & - \\
    % \midrule 
    % {(XXX)}&  City Image & R50 & $\rightarrow^\dagger$& R18                 & 11.4 & 16.4 & 20.3 & 22.8\\
    {(k)}&  City (p)  & R50$^\star$ &$\rightarrow$& R50                    & 4.6 & 6.6 & - & - & - \\
    {(l)}&  City (p)  & R50 &$\rightarrow$& R50                            & 18.0 & 34.0 & 39.8 & 45.6 & 55.5 \\
    {(m)} & City  (p) & R18 (AM) &$\rightarrow^\dagger$& R50x2  & 12.5 & 20.7 & 24.4 & 30.2 & 43.8 \\
    {(n)} & City  (p) & R18 &$\rightarrow^\dagger$& R50x2                 & 46.1 & 55.6 & 59.7 & 63.1 & 69.0 \\
    % {(k)}&  1x City & R50 & $\rightarrow^\dagger$& WR50-2                & 27.3 & 34.2 & 44.2 & 50.5 & 62.2\\
    \bottomrule
  \end{tabu}
% \end{table}




==> kd-single-image (ICLR 2023)/tables/larger_scale.tex <==
% \begin{table}
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \footnotesize
%   \caption{\textbf{Larger scale datasets. Student from IN-1k init.}\label{tab:larger-scale}}
%   \begin{tabular}{l cc c a}
%   \toprule
%      && \multicolumn{3}{c}{\textbf{Student Acc.}} \\
%     & Tchr. Acc. & normal & ours & $\Delta$ \\
%     \midrule 
%     Flowers 102 \\
%     Pets 37 \\
%     Food 101 \\
%     SUN 397 \\
%     \textbf{IN-1k} \\
%     \bottomrule
%   \end{tabular}
% \end{table}
% \begin{table}
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \footnotesize
%   \caption{\textbf{Larger scale datasets. Student from scratch}\label{tab:larger-scale}}
%   \begin{tabular}{ll ll c a}
%   \toprule
%     Dataset & \#Images& Teacher$_\mathrm{Acc}$ & Student$_\mathrm{Acc}$   & Ours  \\
%     \midrule 
%     Pets 37     & 3K  & ResNet-50$_{\,94.03}$ & Resnet-18$_{\,91.42}$\\
%     Flowers 102 & 1K   & ResNet-50$_{\,89.87}$ & Resnet-18$_{\,87.91}$\\
%     Places 365  & 1.8M & ResNet-50$_{\,54.74}$ & Resnet-18$_{\,xx}$\\
%     IN-1k       & 1.3M & ResNet-50$_{\,76.13}$ & Resnet-18$_{\,69.76}$ \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}
\setlength{\tabcolsep}{3pt}
  \centering
  \footnotesize
     \caption{\textbf{Larger scale datasets.}  Teacher is ResNet-18 and student is varied between ResNet-50 and ResNet-50x2.
  Students are trained from scratch. Gap to teacher in brackets for ResNet-50x2. \label{tab:larger-scale}}
  \begin{tabular}{l l ccc}
  \toprule
     &&&  \multicolumn{2}{c}{\textbf{1-Image-Distill}} \\
     \textbf{Dataset} & \textbf{Categories (\#Classes)} & \textbf{Teacher (R18)}  & $\rightarrow$R18 & $\rightarrow$R50x2\\
    \midrule                                                                    % with R18 as teacher:
    STL-10~\citep{pmlr-v15-coates11a}        & Generic objects (10)    &  96.3 &  93.9 & 95.0 (-1.3)\\
    ImageNet-100~\citep{tian2020contrastive} & Objects (100)           &  89.6 & 84.4 & 88.5 (-1.1) \\
    Flowers~\citep{Nilsback06}               & Flower types (102)      &  87.9 & 81.5 & 83.8 (-4.1) \\ 
    Places~\citep{zhou2017places}            & Scenes (365)            &  54.0 & 50.3 & 53.1 (-0.9) \\
    ImageNet~\citep{deng2009imagenet}        & Objects (1000)          &  69.5 & 66.2 & 69.0 (-0.5) \\
    \bottomrule
  \end{tabular}
\end{table}




%%%%%%%%%%%%%%%%%%%%%%% OLD
% \begin{table}
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \footnotesize
%   \begin{tabular}{l l cc}
%   \toprule
%     %  &&&  \multicolumn{1}{c}{\textbf{1-image + Distill}} \\
%      Dataset & Categories (\#Classes) & Teacher  & \textbf{1-image + Distill} \\
%     \midrule                                                                    % with R18 as teacher:
%     STL-10~\citep{pmlr-v15-coates11a} & Generic objects (10)    & 97.8 & 93.0 \\ % 96.3 | 91.9
%     Pets~\citep{parkhi12a}            & Cat \& dog species (37) & 94.0 & 83.7 \\ % 91.4 | 76.9
%     ImageNet-100~\citep{tian2020contrastive} & Objects (100)    & 92.0 & 74.1 \\ % 89.6 | 79.7
%     Flowers~\citep{Nilsback06}        &  Flower types (102)     & 89.8 & 58.1 \\ % 87.9 | 54.1 
%     Places~\citep{zhou2017places}     & Scenes (365)            & 54.7 & 38.2 \\ % 54.0 | 40.5
%     ImageNet~\citep{deng2009imagenet} & Objects (1000)          & 76.1 & 53.5 \\ % 69.5 | 59.1
%     \bottomrule
%   \end{tabular}
%   \vspace{-0.5em}
%   \caption{\textbf{Larger scale datasets.} Both teacher and student are ResNet-50 -- note, however, that this might not be the best setting, see \cref{tab:in1k-analysis}.
%   Teacher models were finetuned from IN-1k pretrained models, students are trained from scratch. \label{tab:larger-scale}}
% \end{table}



==> kd-single-image (ICLR 2023)/tables/other_domain.tex <==
% \begin{table}
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \footnotesize
%   \caption{\textbf{Distilling dataset.} Combining single images works across domains. \todo{WRN40x4-WRN16x4} \label{tab:other}}
%   \vspace{-1em}
%   \begin{tabular}{l rr ccc }
%   \toprule
%   \multicolumn{3}{c}{\textbf{Distillation dataset}} & \multicolumn{3}{c}{\textbf{Accuracy}} \\ 
%   \cmidrule{4-6}
%     Name   & \# Images & \# Pixels & C100 & EuroSAT & PathMNIST\\
%     \midrule 
%     EuroSAT & 21{,}600  & 88M & 9.36 & 97.85 \\
%     CIFAR-100 & 50{,}000  & 51M &  76.26 & 52.24\\
%     PathMNIST & 89{,}996 \\
%     \midrule
%     Image `Animals'  & 1 & 2.8M & 68.69 & 95.04 \\
%     Image `Airport' & 1 & 32M   & 47.44 & 93.46 \\
%     Image `Pathology' & 1 \\
%     % \midrule 
%     % 50\% `Animals' + 50\% `Airport' & 2   & 34.8M & xx & 95.37 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}
\setlength{\tabcolsep}{2pt}
  \centering
  \footnotesize
      \caption{\textbf{Distilling dataset.} Combining single images works across domains. The teacher is a WideR40-4 and the student a WideR16-4 network. \label{tab:other}}
  \begin{tabular}{l rr cc }
  \toprule
  \multicolumn{3}{c}{\textbf{Distillation dataset}} & \multicolumn{2}{c}{\textbf{Accuracy}} \\ 
    Name   & \# Images & \# Pixels & C100 & EuroSAT \\
    \midrule 
    EuroSAT & 21{,}600  & 88M & 9.36 & 97.85 \\
    CIFAR-100 & 50{,}000  & 51M &  76.26 & 52.24\\
    \midrule
    Image ``Animals''  & 1 & 2.8M & 68.69 & 95.04 \\
    Image ``Satellite-pic'' & 1 & 15.7M   & 47.44 & 93.46 \\
    \midrule 
    50\% ``Animals' + 50\% ``Satellite-pic'' & 2   & 19.5M & 66.07 & 95.37 \\
    \bottomrule
  \end{tabular}
\end{table}

==> kd-single-image (ICLR 2023)/tables/representation_exps.tex <==
\begin{table}
% \setlength{\tabcolsep}{pt}
  \centering
  \footnotesize
      \caption{\textbf{Representation learning performance.} 
We compare our distillation approach (R18$\rightarrow$R50) against pretraining via MoCo-v2 on the same data.
We report: linear eval. accuracy on IN-1k and Places; accuracy when finetuning and using $1$\% of ImageNet with labels; SVM classification mAP on PVOC07 and accuracy on Places with varying numbers of images per class; mAP for COCO-detection with FPN. \label{tab:rep}}
  \begin{tabular}{l ccccc ccc }
  \toprule 
     & IN-1k  & Places  & IN-1k (1\%) & \multicolumn{2}{c}{PVOC}  & \multicolumn{2}{c}{Places}   & COCO\\
    \multicolumn{1}{r}{\textit{{ imgs / class}}} &\textit{$\sim$1K}&\textit{$\sim$10K}&\textit{$\sim$13}&  \textit{4} & \textit{16} & \textit{4} & \textit{16} & NA \\
    \midrule
    IN-1k teacher &[69.8] & 44.1 & [69.8] &  65.7 & 77.1  & 21.4 & 30.4 & - \\
    IN-1k R50 & [76.2] & 51.5 & [76.2] & 73.8 & 82.3 & 27.0 & 35.4 & 38.9 \\
    1-image \textbf{MoCo-v2}        & 28.5   & 28.8 & 14.4 & 17.2 & 26.6  & 4.5  & 9.7  & 35.6 \\
    1-image \textbf{Distill}        & 68.8   & 47.2 & 64.1 & 58.9 & 73.5  & 21.0 & 31.3 & 35.4  \\
  % \textbf{Distill}        & 66.1   & 47.1 & 65.2 & 59.4 & 73.5  & 20.6 & 30.8 & 36.3 \\ 
    \bottomrule
  \end{tabular}
\end{table}







% \begin{table}
% \setlength{\tabcolsep}{2pt}
%   \centering
%   \footnotesize
%   \begin{tabular}{l ccccc cc}
%   \toprule 
%     \textbf{1-img Model} & IN-1k  & Places  & IN-1k (1\%) & \multicolumn{2}{c}{PVOC}  & \multicolumn{2}{c}{Places}   \\
%     \multicolumn{1}{r}{\textit{imgs per class}} &\textit{$\sim$1K}&\textit{$\sim$10K}&\textit{$\sim$13}&  \textit{4} & \textit{16} & \textit{4} & \textit{16}  \\
%     \midrule
%     % Fractal pretraining    & 9.2 & 12.6 & 1.5 & 38.7 & 75.8 \\
%     \textbf{MoCo-v2}        & 28.5   & 28.8 & 14.4 & 17.2 & 26.6  & 4.5  & 9.7 \\
%     \textbf{Distill}        & 66.1   & 47.1 & 65.2 & 59.4 & 73.5  & 20.6 & 30.8\\
%     \bottomrule
%   \end{tabular}
%   \vspace{-0.5em}
%     \caption{\textbf{Representation learning performance.} 
% We compare our distillation approach (R50$\rightarrow$R50) against self-supervised pretraining via MoCo-v2 on the same data.
% We report: linear eval. accuracy on IN-1k and Places; accuracy when finetuning and using $1$\% of ImageNet with labels; SVM classification mAP on PVOC07 and accuracy on Places with varying numbers of images per class. \label{tab:rep}}
% \end{table}


==> kd-single-image (ICLR 2023)/tables/vary_archs.tex <==
\begin{table}[tb]
\centering
    \caption{\textbf{Distilling various architectures} on CIFAR-10/100. We compare student accuracy when distilling with full training set vs our 1-image dataset \label{tab:architectures}}
\setlength{\tabcolsep}{4pt}
  \centering
  \footnotesize
  \begin{tabular}{l llc cc cc}
  \toprule
     & &&&\multicolumn{3}{c}{\textbf{Distillation}} \\
     & \textbf{Teacher}$_\mathrm{\qquad Acc.}$  & \textbf{Student}$_\mathrm{\quad \,\,\,\, Acc.}$ && Full & Ours & $\Delta < 5\%$ \\
    \midrule 
    \parbox[t]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\quad \,\,\,\,\,CIFAR10}}} &
    % VGG-19$_{\,\,\quad \,\, 93.28}$    & VGG-11$_{\,\,\,\qquad 92.02}$    && 92.42 & 84.67  \\
    VGG-19$_{\,\,\quad \,\, 93.28}$    & VGG-16$_{\,\,\,\quad 92.42}$  && 92.84 & 92.14 &  \cmarkc \\
    & ResNet-56$_{\,\,\,\,\,93.77}$  & ResNet-20$_{\, \,\,\, 92.52}$ && 92.29 & 90.70  & \cmarkc \\
    %& ResNet-110$_{\,\,93.55}$  & ResNet-56$_{\, \,\,\, 93.77}$ && 92.09 & 90.77  \\
    & WideR40-4$_{\,\,\, 95.42}$& WideR16-4$_{ \,\,   95.20}$ && 95.00 &  93.32 & \cmarkc \\
    & WideR40-4$_{\,\,\, 95.42}$& WideR40-4$_{\,\,95.42}$  & & 94.36 & 94.14 & \cmarkc \\
    & WideR16-4$_{\,\,\, 95.20}$& WideR40-4$_{ \,\,95.42}$ && 94.30 & 94.02 & \cmarkc \\
    \midrule
    \parbox[t]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\quad \, \, \,\,CIFAR100}}} & 
    % VGG-19$_{\,\,\quad \,\, 70.79}$    & VGG-11$_{\,\,\,\qquad 70.71}$    && 72.31 & 56.68  \\
    VGG-19$_{\,\,\quad \,\, 70.79}$    & VGG-16$_{\,\,\,\quad 73.26}$    && 71.19 & 58.66 & \xmarkc   \\
    & ResNet-56$_{\,\,\,\,\,70.99}$  & ResNet-20$_{\, \,\,\, 65.74}$ && 67.04 & 52.43  & \xmarkc  \\
    %& ResNet-110$_{\,\,71.92}$  & ResNet-56$_{\, \,\,\, 70.99}$ && 70.43 & 58.13  \\
    & WideR40-4$_{\,\,\, 78.14}$& WideR16-4$_{ \,\,75.56}$ && 76.26 & 68.69 &  \xmarkc \\
    & WideR40-4$_{\,\,\, 78.14}$& WideR40-4$_{ \,\,78.14}$  & & 75.54  & 73.80 &  \cmarkc \\
    & WideR16-4$_{\,\, \,78.14}$& WideR40-4$_{ \,\,75.56}$ && 76.29 & 74.08 & \cmarkc \\
    \bottomrule
  \end{tabular}
\end{table}

% \begin{table}[tb]
% \centering
% \setlength{\tabcolsep}{4pt}
%   \centering
%   \footnotesize
%       \caption{\textbf{Distilling various architectures} on CIFAR-10. We compare student accuracy when distilling with full training set vs our 1-image dataset. \label{tab:architectures}}
%   \begin{tabular}{l llc cc cc}
%   \toprule
%      & &&&\multicolumn{2}{c}{\textbf{Distillation}} \\
%      & \textbf{Teacher}$_\mathrm{\qquad Acc.}$  & \textbf{Student}$_\mathrm{\quad \,\,\,\, Acc.}$ && Full & Ours  \\
%     \midrule 
%     \parbox[t]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{CIFAR-$10$}}} &
%     % VGG-19$_{\,\,\quad \,\, 93.28}$    & VGG-11$_{\,\,\,\qquad 92.02}$    && 92.42 & 84.67  \\
%     VGG-19$_{\,\,\quad \,\, 93.28}$    & VGG-16$_{\,\,\,\quad 92.42}$    && 92.84 & 92.14  \\
%     & ResNet-56$_{\,\,\,\,\,93.77}$  & ResNet-20$_{\, \,\,\, 92.52}$ && 92.29 & 90.70  \\
%     & ResNet-110$_{\,\,93.55}$  & ResNet-56$_{\, \,\,\, 93.77}$ && 92.09 & 90.77  \\
%     & WideR40-4$_{\,\,\, 95.42}$& WideR16-4$_{ \,\,   95.20}$ && 95.00 &  93.32 \\
%     & WideR40-4$_{\,\,\, 95.42}$& WideR40-4$_{\,\,95.42}$  & & 94.36 & 94.14 \\
%     & WideR16-4$_{\,\,\, 95.20}$& WideR40-4$_{ \,\,95.42}$ && 94.30 & 94.02 \\
%     \midrule
%     \parbox[t]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{CIFAR-$100$}}} & 
%     % VGG-19$_{\,\,\quad \,\, 70.79}$    & VGG-11$_{\,\,\,\qquad 70.71}$    && 72.31 & 56.68  \\
%     VGG-19$_{\,\,\quad \,\, 70.79}$    & VGG-16$_{\,\,\,\quad 73.26}$    && 71.19 & 58.66  \\
%     & ResNet-56$_{\,\,\,\,\,70.99}$  & ResNet-20$_{\, \,\,\, 65.74}$ && 67.04 & 52.43  \\
%     & ResNet-110$_{\,\,71.92}$  & ResNet-56$_{\, \,\,\, 70.99}$ && 70.43 & 58.13  \\
%     & WideR40-4$_{\,\,\, 78.14}$& WideR16-4$_{ \,\,75.56}$ && 76.26 & 68.69 \\
%     & WideR40-4$_{\,\,\, 78.14}$& WideR40-4$_{ \,\,78.14}$  & & 75.54  & 73.80\\
%     & WideR16-4$_{\,\, \,78.14}$& WideR40-4$_{ \,\,75.56}$ && 76.29 & 74.08 \\
%     \bottomrule
%   \end{tabular}
% \end{table}


==> kd-single-image (ICLR 2023)/tables/vary_distillation_data.tex <==
% \vspace{-0.5em}
% \begin{table}[!htbp]
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \footnotesize
%       \caption{\textbf{Teacher signal.} Even with only top-5 predictions (class \& probability) or hard distillation, performance only slightly degrades. Same setup as in \cref{tab:ablation}
%   \label{tab:dist_type}}
%   \begin{tabular}{l ccc}
%   \toprule 
%                 & Full output &  Top-5 & Argmax \\
%     \midrule
%     \textbf{C10 Accuracy} & 93.32 & 92.98 & 91.89 \\
%     \textbf{C100 Accuracy} & 68.69 &  64.72 & 60.75 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}[!htbp]
\setlength{\tabcolsep}{6pt}
  \centering
  \footnotesize
          \caption{\textbf{Comparison against other datasets on CIFAR-10.} Here the teacher model is WideR40-2 and student is WideR40-1 for comparability to~\citep{Micaelli2019ZeroShotKT}.
    \label{tab:baselines}}
    \begin{tabular}{@{}ccccc@{}}
    \toprule
    \multicolumn{1}{c}{\textbf{CIFAR-10}} & \textbf{Fractals} & \textbf{StyleGAN} & \textbf{ZeroSKD} & \textbf{1-Image (Ours)} \\
    \midrule
       92.61 & 33.26 & 83.42 & 86.60 & 89.27 \\
       \bottomrule
    \end{tabular}
\end{table}

%  94.71 teacher

==> kd-single-image (ICLR 2023)/tables/video.tex <==
% \begin{table}[tb]
  \caption{\textbf{Scaling to video.} Student models are trained from scratch. Top-1 accuracy is shown with 10-temporal center-cropped clips per video. Details in~\cref{app:video}  \label{tab:larger-scale-video}}
\setlength{\tabcolsep}{4pt}
  \centering
  \footnotesize
  \begin{tabular}{l  cc}
  \toprule
     Dataset & Teacher  & \textbf{Distill} \\
    \midrule 
    UCF-101    & 90.4 & 75.2 \\
    K400              & 67.8 & 51.8 \\ %47.86  \\ 
    \bottomrule
  \end{tabular}
% \end{table}
% \begin{table}[tb]
%   \caption{\textbf{Scaling to video.} Student models are trained from scratch. Top-1 accuracy is shown with 10-temporal center-cropped clips per video. Details in~\cref{app:video}  \label{tab:larger-scale-video}}
% \setlength{\tabcolsep}{4pt}
%   \centering
%   \footnotesize
%   \begin{tabular}{l l cc}
%   \toprule
%      Dataset  & Categories (\#Classes) & Teacher  & \textbf{1-image + Distill} \\
%     \midrule 
%     UCF-101~\citep{soomro2012ucf101}     & Human actions (101)      & 90.4 & 75.2 \\
%     K400~\citep{carreira2017quo}         & Human actions (400)      & 67.8 & 51.8 \\ %47.86  \\ 
%     \bottomrule
%   \end{tabular}
% \end{table}

==> tables/_vary_source_size.tex <==
% \begin{table}
\setlength{\tabcolsep}{2pt}
   \centering
   \footnotesize
  \def\arraystretch{1.18}
  \begin{tabular}{l r cc }
  \toprule 
   \multicolumn{1}{c}{\textbf{Training}}& \multicolumn{2}{c}{\textbf{Accuracy}} \\
    Size & C10 & C100\\
    \midrule
    % 50    & 1M  & 30.0 & 5.25 \\
    500    & 92.31 & 58.95\\
    5K     & 93.01 & 63.84\\
    50K    & 93.28 & 66.12\\
    500K   & 93.52 & 67.05\\
    \bottomrule
  \end{tabular}
   \caption{\textbf{Source dataset size.} A larger initial pool is better. \label{tab:abl:size}}
% \end{table}

==> tables/other_domain.tex <==
% \begin{table}
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \footnotesize
%   \caption{\textbf{Distilling dataset.} Combining single images works across domains. \todo{WRN40x4-WRN16x4} \label{tab:other}}
%   \vspace{-1em}
%   \begin{tabular}{l rr ccc }
%   \toprule
%   \multicolumn{3}{c}{\textbf{Distillation dataset}} & \multicolumn{3}{c}{\textbf{Accuracy}} \\ 
%   \cmidrule{4-6}
%     Name   & \# Images & \# Pixels & C100 & EuroSAT & PathMNIST\\
%     \midrule 
%     EuroSAT & 21{,}600  & 88M & 9.36 & 97.85 \\
%     CIFAR-100 & 50{,}000  & 51M &  76.26 & 52.24\\
%     PathMNIST & 89{,}996 \\
%     \midrule
%     Image `Animals'  & 1 & 2.8M & 68.69 & 95.04 \\
%     Image `Airport' & 1 & 32M   & 47.44 & 93.46 \\
%     Image `Pathology' & 1 \\
%     % \midrule 
%     % 50\% `Animals' + 50\% `Airport' & 2   & 34.8M & xx & 95.37 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}
\setlength{\tabcolsep}{2pt}
  \centering
  \footnotesize
      \caption{\textbf{Distilling dataset.} Combining single images works across domains. The teacher is a WideR40-4 and the student a WideR16-4 network. \label{tab:other}}
  \begin{tabular}{l rr cc }
  \toprule
  \multicolumn{3}{c}{\textbf{Distillation dataset}} & \multicolumn{2}{c}{\textbf{Accuracy}} \\ 
    Name   & \# Images & \# Pixels & C100 & EuroSAT \\
    \midrule 
    EuroSAT & 21{,}600  & 88M & 9.36 & 97.85 \\
    CIFAR-100 & 50{,}000  & 51M &  76.26 & 52.24\\
    \midrule
    Image ``Animals''  & 1 & 2.8M & 68.69 & 95.04 \\
    Image ``Satellite-pic'' & 1 & 15.7M   & 47.44 & 93.46 \\
    \midrule 
    50\% ``Animals' + 50\% ``Satellite-pic'' & 2   & 19.5M & 66.07 & 95.37 \\
    \bottomrule
  \end{tabular}
\end{table}

==> tables/vary_distillation_data.tex <==
% \vspace{-0.5em}
% \begin{table}[!htbp]
% \setlength{\tabcolsep}{3pt}
%   \centering
%   \footnotesize
%       \caption{\textbf{Teacher signal.} Even with only top-5 predictions (class \& probability) or hard distillation, performance only slightly degrades. Same setup as in \cref{tab:ablation}
%   \label{tab:dist_type}}
%   \begin{tabular}{l ccc}
%   \toprule 
%                 & Full output &  Top-5 & Argmax \\
%     \midrule
%     \textbf{C10 Accuracy} & 93.32 & 92.98 & 91.89 \\
%     \textbf{C100 Accuracy} & 68.69 &  64.72 & 60.75 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}[!htbp]
\setlength{\tabcolsep}{6pt}
  \centering
  \footnotesize
          \caption{\textbf{Comparison against other datasets on CIFAR-10.} Here the teacher model is WideR40-2 and student is WideR40-1 for comparability to~\citep{Micaelli2019ZeroShotKT}.
    \label{tab:baselines}}
    \begin{tabular}{@{}ccccc@{}}
    \toprule
    \multicolumn{1}{c}{\textbf{CIFAR-10}} & \textbf{Fractals} & \textbf{StyleGAN} & \textbf{ZeroSKD} & \textbf{1-Image (Ours)} \\
    \midrule
       92.61 & 33.26 & 83.42 & 86.60 & 89.27 \\
       \bottomrule
    \end{tabular}
\end{table}

%  94.71 teacher
